Beyond Individualized Recourse: Interpretable and Interactive Summaries of Actionable Recourses

As predictive models are increasingly being deployed in high-stakes decision-making, there has been a lot of interest in developing algorithms which can provide recourses to affected individuals. While developing such tools is important, it is even more critical to analyse and interpret a predictive model, and vet it thoroughly to ensure that the recourses it offers are meaningful and non-discriminatory before it is deployed in the real world. To this end, we propose a novel model agnostic framework called Actionable Recourse Summaries (AReS) to construct global counterfactual explanations which provide an interpretable and accurate summary of recourses for the entire population. We formulate a novel objective which simultaneously optimizes for correctness of the recourses and interpretability of the explanations, while minimizing overall recourse costs across the entire population. More specifically, our objective enables us to learn, with optimality guarantees on recourse correctness, a small number of compact rule sets each of which capture recourses for well defined subpopulations within the data. We also demonstrate theoretically that several of the prior approaches proposed to generate recourses for individuals are special cases of our framework. Experimental evaluation with real world datasets and user studies demonstrate that our framework can provide decision makers with a comprehensive overview of recourses corresponding to any black box model, and consequently help detect undesirable model biases and discrimination.

==> Submission/uncertainty-sampling-algo.tex <==
\begin{algorithm}
  \caption{Uncertainty sampling for local explanations
    \label{alg:uncertainty-sampling-local-explanations}}
  \begin{algorithmic}[1]
    \Require{Perturbation size $N$, Batch size $B$, Model $f$, Data instance $X$, Explanation Model $g$ with Predictive Variance $\phi_g$, Candidate perturbation batch size $\mathcal{A}$}
    % \Statex
    
    % \hspace{6mm} \State{Let $f(\cdot)$ be the model prediction operation.}
    
    % \Let{Let $g^*(\cdot)$ be the predictive uncertainty operation.}

    \Function{Uncertainty sample}{$N, B, f, g$}
    
    \State{Initialize data set $\mathcal{D}$ and add a small number of local perturbations, $(\mathcal{Z},f(\mathcal{Z}))$.}
    
    \State{Fit $g$ on $\mathcal{D}$}
    
      \For{$i \gets 1 \textrm{ to } N - |\mathcal{Z}|$}
        \If{$i$ \textrm{mod.} $B = 0$}
         
        %  \hspace{10mm} 
         \State{Generate set of candidate perturbations $\mathcal{Q}$ of size $\mathcal{A}$}
         
        %  \hspace{10mm} 
         \State{Draw $B$ perturbations into $\mathcal{Q_{\textrm{new}}}$ from 
        %  \hspace{30mm}
         $\mathcal{Q}_{\textrm{dist}} \sim \exp(\phi_g(\mathcal{Q}))_{j\in|\mathcal{Q}|} / \sum\exp(\phi_g(\mathcal{Q})) $}
         
        %   \hspace{10mm} 
          \State{$\mathcal{D}\gets \mathcal{D}\cup (\mathcal{Q_{\textrm{new}}}, f(\mathcal{Q}_\textrm{new})); $ Fit $g$ on $ \mathcal{D}$}
         
        \EndIf
    
      \EndFor
      \State \Return{$g$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}
